Improving Graph Convolutional Networks with Transformer Layer in social-based items recommendation

In this work, we have proposed an approach for improving the GCN for predicting ratings in social networks. Our model is expanded from the standard model with several layers of transformer architecture. The main focus of the paper is on the encoder architecture for node embedding in the network. Using the embedding layer from the graph-based convolution layer, the attention mechanism could rearrange the feature space to get a more efficient embedding for the downstream task. The experiments showed that our proposed architecture achieves better performance than GCN on the traditional link prediction task.

==> tables/predict_table.tex <==
\begin{table*}[!htbp]
    \centering
    \caption{Example of rating are predicted by different recommender algorithms}
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{ |c|c|c|c|c|c|c|c| }

        \hline
         \textbf{UserId} & \textbf{ItemId} & \textbf{Rating} & \textbf{PMF} & \textbf{NeuMF} & \textbf{Graph} \par \textbf{Rec} & \textbf{GCN} & \textbf{GTN(our model)}\\
        \hline
         6636 & 64244 & 4 & 3.54 & 3.70 & 4.12 & 3.82 & 3.91\\
        \hline
         585  & 3842 & 5 & 4.01 & 4.53 & 4.49 & 4.34 & 4.24    \\
        \hline
        582 & 2102 & 3 & 3.67 & 3.78 & 4.05 & 3.21 & 2.9 \\
        \hline
        208 & 17554 & 2 & 3.52 & 2.57 & 4.30 & 3.43 & 3.21 \\
        \hline
        1 & 503 & 5 & 3.49 & 3.99 & 4.19 & 3.84 & 4.34 \\
        \hline
    \end{tabular}
    \end{adjustbox}
\end{table*}

